Active Weighted Aging Ensemble for Drifted Data Stream Classification

One of the significant problems of streaming data classification is the occurrence of concept drift, consisting of the change of probabilistic characteristics of the classification task. This phenomenon destabilizes the performance of the classification model and seriously degrades its quality. An appropriate strategy counteracting this phenomenon is required to adapt the classifier to the changing probabilistic characteristics. One of the significant problems in implementing such a solution is the access to data labels. It is usually costly, so to minimize the expenses related to this process, learning strategies based on semi-supervised learning are proposed, e.g., employing active learning methods indicating which of the incoming objects are valuable to be labeled for improving the classifier's performance. This paper proposes a novel chunk-based method for non-stationary data streams based on classifier ensemble learning and an active learning strategy considering a limited budget that can be successfully applied to any data stream classification algorithm. The proposed method has been evaluated through computer experiments using both real and generated data streams. The results confirm the high quality of the proposed algorithm over state-of-the-art methods.

==> tables/table_post_pruning_aging_method.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{tabularx}{\columnwidth}{cc|CCC|CCC|CCC}
\toprule

& &\multicolumn{3}{c|}{\bfseries GNB} & \multicolumn{3}{c|}{\bfseries HT} & \multicolumn{3}{c}{\bfseries MLP} \\
& & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c}{\textsc{gauss}} \\ \midrule


\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}
& \textsc{post} & \bfseries 0.839 & 0.815 & 0.736 & \bfseries 0.839 & 0.815 & 0.74  & \bfseries 0.908 & 0.879 & 0.812 \\
& \textsc{pre} & \bfseries 0.838 & 0.814 & 0.727 & \bfseries 0.839 & 0.814 & 0.724 & \bfseries 0.908 & 0.878 & 0.804 \\\midrule


\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{grad.}}}
& \textsc{post} & \bfseries 0.829 & 0.811 & 0.752 & \bfseries 0.829 & 0.811 & 0.755 & \bfseries 0.918 & 0.895 & 0.851 \\
& \textsc{pre} & \bfseries 0.827 & 0.810  & 0.752 & \bfseries 0.827 & 0.810  & 0.751 & \bfseries 0.916 & 0.893 & 0.841 \\\midrule


\multirow{2}{*}{\rotatebox[origin=c]{90}{\textsc{inc.}}}
& \textsc{post} & \bfseries 0.862 & 0.841 & 0.778 & \bfseries 0.862 & 0.841 & 0.773 & \bfseries 0.925 & 0.900   & 0.829 \\
& \textsc{pre} & \bfseries 0.861 & 0.84  & 0.775 & \bfseries 0.860 & 0.839 & 0.768 & \bfseries 0.922 & 0.898 & 0.823 \\
\bottomrule
\end{tabularx}

==> tables/table_post_pruning_theta.tex <==
\renewcommand{\arraystretch}{1.25}

\begin{tabularx}{\columnwidth}{cC|CC|CC|CC}
\toprule
& &\multicolumn{2}{c|}{\bfseries GNB} & \multicolumn{2}{c|}{\bfseries HT} & \multicolumn{2}{c}{\bfseries MLP} \\
& & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c|}{\textsc{pre}} & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c|}{\textsc{pre}} & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c}{\textsc{pre}} \\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}

&{\tiny $0\%$}& \bfseries 0.796 & 0.791       & \bfseries 0.798 & 0.791       & 0.864       & 0.861       \\
&{\tiny $2.5\%$}& \bfseries 0.801 & \bfseries 0.798 & \bfseries 0.803 & 0.797       & \bfseries 0.871 & \bfseries 0.869 \\
&{\tiny $5\%$}& \bfseries 0.804 & \bfseries 0.800 & \bfseries 0.806 & \bfseries 0.800 & \bfseries 0.875 & \bfseries 0.873 \\
&{\tiny $7.5\%$}& \bfseries 0.805 & \bfseries 0.801 & \bfseries 0.806 & \bfseries 0.801 & \bfseries 0.877 & \bfseries 0.874 \\
&{\tiny $10\%$}& 0.777       & 0.773       & 0.778       & 0.773       & 0.843       & 0.840       \\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{gradual}}}

&{\tiny $0\%$}& \bfseries 0.799 & \bfseries 0.797 & \bfseries 0.800 & 0.797       & \bfseries 0.892 & 0.886       \\
&{\tiny $2.5\%$}& \bfseries 0.802 & \bfseries 0.801 & \bfseries 0.803 & \bfseries 0.801 & \bfseries 0.895 & \bfseries 0.890 \\
&{\tiny $5\%$}& \bfseries 0.804 & \bfseries 0.803 & \bfseries 0.805 & \bfseries 0.802 & \bfseries 0.896 & \bfseries 0.891 \\
&{\tiny $7.5\%$}& \bfseries 0.805 & \bfseries 0.804 & \bfseries 0.806 & \bfseries 0.804 & \bfseries 0.896 & \bfseries 0.892 \\
&{\tiny $10\%$}& 0.778       & 0.777       & 0.779       & 0.777       & 0.862       & 0.858       \\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{incremental}}}

&{\tiny $0\%$}& \bfseries 0.829 & 0.826       & \bfseries 0.827 & 0.823       & 0.886       & 0.881       \\
&{\tiny $2.5\%$}& \bfseries 0.833 & \bfseries 0.830 & \bfseries 0.831 & \bfseries 0.828 & \bfseries 0.891 & \bfseries 0.887 \\
&{\tiny $5\%$}& \bfseries 0.834 & \bfseries 0.832 & \bfseries 0.832 & \bfseries 0.829 & \bfseries 0.893 & \bfseries 0.889 \\
&{\tiny $7.5\%$}& \bfseries 0.835 & \bfseries 0.833 & \bfseries 0.833 & \bfseries 0.831 & \bfseries 0.894 & \bfseries 0.891 \\
&{\tiny $10\%$}& 0.805       & 0.804       & 0.803       & 0.801       & 0.859       & 0.856       \\
\bottomrule
\end{tabularx}

==> tables/table_post_pruning_weight_calculation_method.tex <==
\renewcommand{\arraystretch}{1.25}

\begin{tabularx}{\columnwidth}{cC|CC|CC|CC}
\toprule
& &\multicolumn{2}{c|}{\bfseries GNB} & \multicolumn{2}{c|}{\bfseries HT} & \multicolumn{2}{c}{\bfseries MLP} \\
& & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c|}{\textsc{pre}} & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c|}{\textsc{pre}} & \multicolumn{1}{c}{\textsc{post}} & \multicolumn{1}{c}{\textsc{pre}} \\\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}

& \textsc{same} & 0.764       & 0.757       & 0.768       & 0.758       & 0.834       & 0.830       \\
& \textsc{kunch.} & \bfseries 0.836 & \bfseries 0.835 & \bfseries 0.836 & \bfseries 0.834 & \bfseries 0.908 & \bfseries 0.908 \\
& \textsc{pta} & 0.799       & 0.796       & 0.799       & 0.794       & 0.871       & 0.869       \\
& \textsc{bell} & 0.788       & 0.784       & 0.789       & 0.783       & 0.851       & 0.846       \\\midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{grad.}}}
 & \textsc{same} & 0.782       & 0.781       & 0.785       & 0.782       & 0.883       & 0.876       \\
& \textsc{kunch.} & \bfseries 0.816 & \bfseries 0.815 & \bfseries 0.816 & \bfseries 0.815 & \bfseries 0.899 & \bfseries 0.896 \\
& \textsc{pta} & 0.796       & 0.796       & 0.797       & 0.795       & 0.889       & 0.884       \\
& \textsc{bell} & 0.795       & 0.793       & 0.796       & 0.793       & 0.881       & 0.877       \\\midrule
 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{inc.}}}
& \textsc{same} & 0.810       & 0.808       & 0.808       & 0.802       & 0.864       & 0.861       \\
& \textsc{kunch.} & \bfseries 0.848 & \bfseries 0.847 & \bfseries 0.847 & \bfseries 0.846 & \bfseries 0.910 & \bfseries 0.907 \\
& \textsc{pta} & 0.827       & 0.825       & 0.823       & 0.822       & 0.886       & 0.883       \\
& \textsc{bell} & 0.824       & 0.820       & 0.823       & 0.820       & 0.879       & 0.873       \\
\bottomrule
\end{tabularx}

==> tables/table_theta_aging_method.tex <==
\renewcommand{\arraystretch}{1.3}

\begin{tabularx}{\columnwidth}{cC|CCC|CCC|CCC}
\toprule
& &\multicolumn{3}{c|}{\bfseries GNB} & \multicolumn{3}{c|}{\bfseries HT} & \multicolumn{3}{c}{\bfseries MLP} \\

& & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c}{\textsc{gauss}}\\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}

&{\tiny $0\%$}&\bfseries 0.839 & 0.811       & 0.731 & \bfseries 0.839 & 0.812       & 0.732 & \bfseries 0.908 & 0.872       & 0.808 \\
&{\tiny $2.5\%$}&\bfseries 0.839 & 0.828       & 0.731 & \bfseries 0.839 & 0.829       & 0.732 & \bfseries 0.908 & 0.894       & 0.808 \\
&{\tiny $5\%$}&\bfseries 0.839 & \bfseries 0.837 & 0.731 & \bfseries 0.839 & \bfseries 0.837 & 0.732 & \bfseries 0.908 & \bfseries 0.906 & 0.808 \\
&{\tiny $7.5\%$}&\bfseries 0.839 & \bfseries 0.839 & 0.731 & \bfseries 0.839 & \bfseries 0.839 & 0.732 & \bfseries 0.908 & \bfseries 0.910 & 0.808 \\
&{\tiny $10\%$}&\bfseries 0.839 & 0.755       & 0.731 & \bfseries 0.839 & 0.755       & 0.732 & \bfseries 0.908 & 0.808       & 0.808 \\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{gradual}}}
 
&{\tiny $0\%$}&\bfseries 0.828 & 0.813       & 0.752 & \bfseries 0.828 & 0.813       & 0.753 & \bfseries 0.917 & 0.903       & 0.846 \\
&{\tiny $2.5\%$}&\bfseries 0.828 & \bfseries 0.825 & 0.752 & \bfseries 0.828 & \bfseries 0.825 & 0.753 & \bfseries 0.917 & \bfseries 0.913 & 0.846 \\
&{\tiny $5\%$}&\bfseries 0.828 & \bfseries 0.830 & 0.752 & \bfseries 0.828 & \bfseries 0.830 & 0.753 & \bfseries 0.917 & \bfseries 0.917 & 0.846 \\
&{\tiny $7.5\%$}&\bfseries 0.828 & \bfseries 0.833 & 0.752 & \bfseries 0.828 & \bfseries 0.833 & 0.753 & \bfseries 0.917 & \bfseries 0.919 & 0.846 \\
&{\tiny $10\%$}&\bfseries 0.828 & 0.752       & 0.752 & \bfseries 0.828 & 0.752       & 0.753 & \bfseries 0.917 & 0.817       & 0.846 \\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{incremental}}}
 
&{\tiny $0\%$}&\bfseries 0.862 & 0.844       & 0.776 & \bfseries 0.861 & 0.844       & 0.771 & \bfseries 0.924 & 0.900       & 0.826 \\
&{\tiny $2.5\%$}&\bfseries 0.862 & 0.857       & 0.776 & \bfseries 0.861 & \bfseries 0.856 & 0.771 & \bfseries 0.924 & 0.918       & 0.826 \\
&{\tiny $5\%$}&\bfseries 0.862 & \bfseries 0.862 & 0.776 & \bfseries 0.861 & \bfseries 0.861 & 0.771 & \bfseries 0.924 & \bfseries 0.924 & 0.826 \\
&{\tiny $7.5\%$}&\bfseries 0.862 & \bfseries 0.865 & 0.776 & \bfseries 0.861 & \bfseries 0.864 & 0.771 & \bfseries 0.924 & \bfseries 0.929 & 0.826 \\
&{\tiny $10\%$}&\bfseries 0.862 & 0.775       & 0.776 & \bfseries 0.861 & 0.775       & 0.771 & \bfseries 0.924 & 0.824       & 0.826 \\
\bottomrule
\end{tabularx}

==> tables/table_theta_weight_calculation_method.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{tabularx}{\textwidth}{cC|CCCC|CCCC|CCCC}

\toprule
& &\multicolumn{4}{c|}{\bfseries GNB} & \multicolumn{4}{c|}{\bfseries HT} & \multicolumn{4}{c}{\bfseries MLP} \\

& & \multicolumn{1}{c}{\textsc{same}} & \multicolumn{1}{c}{\textsc{kun.}} & \multicolumn{1}{c}{\textsc{pta}} & \multicolumn{1}{c|}{\textsc{bell}}
& \multicolumn{1}{c}{\textsc{same}} & \multicolumn{1}{c}{\textsc{kun.}} & \multicolumn{1}{c}{\textsc{pta}} & \multicolumn{1}{c|}{\textsc{bell}}
& \multicolumn{1}{c}{\textsc{same}} & \multicolumn{1}{c}{\textsc{kun.}} & \multicolumn{1}{c}{\textsc{pta}} & \multicolumn{1}{c}{\textsc{bell}}\\\midrule

\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}


&{\scriptsize $0\%$}&0.755 & \bfseries 0.835 & 0.793 & 0.792       & 0.758 & \bfseries 0.835 & 0.792 & 0.793       & 0.825 & \bfseries 0.908 & 0.864 & 0.854       \\
&{\scriptsize $2.5\%$}&0.757 & \bfseries 0.835 & 0.795 & 0.809       & 0.760  & \bfseries 0.835 & 0.795 & 0.810       & 0.828 & \bfseries 0.908 & 0.868 & 0.877       \\
&{\scriptsize $5\%$}&0.761 & \bfseries 0.835 & 0.797 & 0.815       & 0.763 & \bfseries 0.835 & 0.797 & 0.816       & 0.832 & \bfseries 0.908 & 0.870  & 0.885       \\
&{\scriptsize $7.5\%$}&0.763 & \bfseries 0.836 & 0.799 & 0.815       & 0.766 & \bfseries 0.835 & 0.799 & 0.815       & 0.836 & \bfseries 0.908 & 0.873 & 0.884       \\
&{\scriptsize $10\%$}&0.766 & \bfseries 0.836 & 0.801 & 0.697       & 0.769 & \bfseries 0.835 & 0.800   & 0.697       & 0.841 & \bfseries 0.908 & 0.875 & 0.742       \\\midrule
 
 
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{gradual}}}
&{\scriptsize $0\%$}&0.778 & \bfseries 0.814 & 0.793 & 0.807       & 0.780  & \bfseries 0.813 & 0.792 & 0.808       & 0.876 & 0.896       & 0.883 & 0.900       \\
&{\scriptsize $2.5\%$}&0.78  & \bfseries 0.815 & 0.795 & \bfseries 0.818 & 0.781 & \bfseries 0.815 & 0.794 & \bfseries 0.819 & 0.877 & 0.897       & 0.885 & \bfseries 0.909 \\
&{\scriptsize $5\%$}&0.782 & \bfseries 0.816 & 0.796 & \bfseries 0.819 & 0.783 & \bfseries 0.816 & 0.796 & \bfseries 0.819 & 0.879 & 0.898       & 0.886 & \bfseries 0.909 \\
&{\scriptsize $7.5\%$}&0.784 & \bfseries 0.817 & 0.798 & \bfseries 0.819 & 0.785 & \bfseries 0.817 & 0.798 & \bfseries 0.819 & 0.881 & 0.899       & 0.888 & \bfseries 0.908 \\
&{\scriptsize $10\%$}&0.786 & \bfseries 0.818 & 0.800   & 0.706       & 0.788 & \bfseries 0.817 & 0.799 & 0.707       & 0.883 & 0.899       & 0.890  & 0.768       \\\midrule
 
 
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textsc{incremental}}}
&{\scriptsize $0\%$}&0.805 & \bfseries 0.846 & 0.822 & 0.837       & 0.801 & \bfseries 0.844 & 0.819 & 0.837       & 0.857 & \bfseries 0.907 & 0.879 & 0.890       \\
&{\scriptsize $2.5\%$}&0.807 & \bfseries 0.847 & 0.824 & \bfseries 0.849 & 0.803 & \bfseries 0.845 & 0.821 & \bfseries 0.848 & 0.859 & \bfseries 0.908 & 0.882 & \bfseries 0.908 \\
&{\scriptsize $5\%$}&0.809 & \bfseries 0.848 & 0.826 & \bfseries 0.850 & 0.805 & \bfseries 0.846 & 0.823 & \bfseries 0.849 & 0.862 & \bfseries 0.909 & 0.885 & \bfseries 0.910 \\
&{\scriptsize $7.5\%$}&0.811 & \bfseries 0.848 & 0.828 & \bfseries 0.850 & 0.807 & \bfseries 0.847 & 0.824 & \bfseries 0.848 & 0.866 & \bfseries 0.909 & 0.887 & \bfseries 0.909 \\
&{\scriptsize $10\%$}&0.813 & \bfseries 0.849 & 0.83  & 0.726       & 0.809 & \bfseries 0.848 & 0.826 & 0.726       & 0.869 & \bfseries 0.910 & 0.889 & 0.763       \\
\bottomrule
\end{tabularx}

==> tables/table_weight_calculation_method_aging_method.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{tabularx}{\columnwidth}{cC|CCC|CCC|CCC}
\toprule

& &\multicolumn{3}{c|}{\bfseries GNB} & \multicolumn{3}{c|}{\bfseries HT} & \multicolumn{3}{c}{\bfseries MLP} \\
& & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c|}{\textsc{gauss}} & \multicolumn{1}{c}{\textsc{prop}} & \multicolumn{1}{c}{\textsc{const}} & \multicolumn{1}{c}{\textsc{gauss}} \\ \midrule

\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{sudden}}}

&\textsc{same}&\bfseries 0.839 & 0.813       & 0.629 & \bfseries 0.839 & 0.815       & 0.636 & \bfseries 0.908 & 0.875       & 0.714 \\
 &\textsc{kunch.}&\bfseries 0.839 & \bfseries 0.842 & 0.825 & \bfseries 0.839 & \bfseries 0.842 & 0.823 & \bfseries 0.908 & \bfseries 0.915 & 0.902 \\
&\textsc{pta}&\bfseries 0.839 & 0.832       & 0.721 & \bfseries 0.839 & 0.832       & 0.719 & \bfseries 0.908 & 0.900       & 0.801 \\
&\textsc{bell}&\bfseries 0.839 & 0.769       & 0.749 & \bfseries 0.839 & 0.770       & 0.75  & \bfseries 0.908 & 0.823       & 0.815 \\\midrule
 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{grad.}}}
 
&\textsc{same}&\bfseries 0.828 & 0.820       & 0.697 & \bfseries 0.828 & 0.820       & 0.702 & \bfseries 0.917 & \bfseries 0.911 & 0.81  \\
&\textsc{kunch.}&\bfseries 0.828 & \bfseries 0.831 & 0.788 & \bfseries 0.828 & \bfseries 0.831 & 0.787 & \bfseries 0.917 & \bfseries 0.915 & 0.861 \\
&\textsc{pta}&\bfseries 0.828 & \bfseries 0.825 & 0.736 & \bfseries 0.828 & \bfseries 0.825 & 0.735 & \bfseries 0.917 & \bfseries 0.914 & 0.829 \\
&\textsc{bell}&\bfseries 0.828 & 0.767       & 0.787 & \bfseries 0.828 & 0.766       & 0.789 & \bfseries 0.917 & 0.836       & 0.883 \\
\midrule
 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textsc{inc.}}}
 
&\textsc{same}&\bfseries 0.862 & 0.851       & 0.714 & \bfseries 0.861 & 0.851       & 0.703 & \bfseries 0.924 & 0.909       & 0.755 \\
&\textsc{kunch.}&\bfseries 0.862 & \bfseries 0.862 & 0.819 & \bfseries 0.861 & \bfseries 0.861 & 0.817 & \bfseries 0.924 & \bfseries 0.925 & 0.877 \\
&\textsc{pta}&\bfseries 0.862 & \bfseries 0.857 & 0.76  & \bfseries 0.861 & \bfseries 0.857 & 0.75  & \bfseries 0.924 & 0.918       & 0.811 \\
&\textsc{bell}&\bfseries 0.862 & 0.792       & 0.812 & \bfseries 0.861 & 0.791       & 0.813 & \bfseries 0.924 & 0.843       & 0.861 \\
\bottomrule
\end{tabularx}

==> tables/wae_optimization.tex <==
\renewcommand{\arraystretch}{1.5}

\begin{tabularx}{\columnwidth}{rlCCCCC}
\toprule

& \bfseries Drift type & \bfseries Accuracy & \bfseries Pruning & \bfseries $\theta$ & \bfseries \textsc{wcm} & \bfseries Aging

\\\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textsc{gnb}}}
&        \textsc{sudden}  &  0.858  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
 &       \textsc{gradual}  &  0.843  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
&   \textsc{incremental}  &  0.876  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textsc{ht}}}
&        \textsc{sudden}  &  0.858  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
 &       \textsc{gradual}  &  0.841  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
&   \textsc{incremental}  &  0.873  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textsc{mlp}}}
 &        \textsc{sudden}  &  0.934  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
 &       \textsc{gradual}  &  0.928  &  ---  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\
 &   \textsc{incremental}  &  0.944  &  \textsc{pre}/\textsc{post}  &  5\%  &  \textsc{bell}  &  \textsc{const}  \\\bottomrule

    \end{tabularx}
